Search for pair production of heavy vector-like quarks decaying to high-$p_{\text{T}}$ $W$ bosons and $b$ quarks in the lepton-plus-jets final state in $pp$ collisions at $\sqrt{s}$=13 TeV with the ATLAS detector

A search is presented for the pair production of heavy vector-like $T$ and $B$ quarks, primarily targeting the $T$ quark decays to a $W$ boson and a $b$-quark. The search is based on $36.1$ fb$^{-1}$ of $pp$ collisions at $\sqrt{s}$ = 13 TeV recorded in 2015 and 2016 with the ATLAS detector at the CERN Large Hadron Collider. Data are analysed in the lepton-plus-jets final state, including at least one $b$-tagged jet and a large-radius jet identified as originating from the hadronic decay of a high-momentum $W$ boson. No significant deviation from the Standard Model expectation is observed in the reconstructed $T$ mass distribution. The observed 95% confidence level lower limit on the $T$ mass are 1350 GeV assuming 100% branching ratio to $Wb$. In the SU(2) singlet scenario, the lower mass limit is 1170 GeV. This search is also sensitive to a heavy vector-like $B$ quark decaying to $Wt$ and other final states. The results are thus reinterpreted to provide a 95% confidence level lower limit on the $B$ quark mass at 1250 GeV assuming 100% branching ratio to $Wt$; in the SU(2) singlet scenario, the limit is 1080 GeV. Mass limits on both $T$ and $B$ production are also set as a function of the decay branching ratios. The 100% branching ratio limits are found to be applicable to heavy vector-like $Y$ and $X$ production that decay to $Wb$ and $Wt$, respectively.

==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $$file"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf


==> commands.tex <==

% Shorthand for \phantom to use in tables
\newcommand{\pho}{\phantom{0}}
\newcommand{\bslash}{\ensuremath{\backslash}}
\newcommand{\BibTeX}{{\sc Bib\TeX}}
\newcommand{\Nl}{\mbox{$N_{\rm{loose}}$}}
\newcommand{\Nt}{\mbox{$N_{\rm{tight}}$}}
\newcommand{\Ns}{\mbox{$N^{\rm{SIG}}$}}
\newcommand{\Nf}{\mbox{$N^{\rm{FAKE}}$}}
\newcommand{\epss}{\mbox{$\varepsilon^{\rm{SIG}}$}}
%\newcommand{\epsf}{\mbox{$\varepsilon^{\rm{FAKE}}$}}
\newcommand{\zmumu}{\mbox{$\rm{Z}^0 \rightarrow \mu \mu$}~}
\newcommand{\zee}{\mbox{$\rm{Z}^0 \rightarrow e e$}~}
\newcommand{\ZZero}{\mbox{$\rm{Z}^0$}~}
\newcommand{\MTW}{\mbox{$M_{\rm{T}}(\rm{W})$}~}
\newcommand{\ljets}{\ensuremath{\ell{}+\text{jets}}}
%\newcommand{\ejets}{\ensuremath{e+\text{jets}}}
\newcommand{\ejets}{$e$+jets}
%\newcommand{\mujets}{\ensuremath{\mu{}+\text{jets}}}
\newcommand{\mujets}{$\mu{}$+jets}

\newcommand{\ECF}{\ensuremath{D_2^{\beta=1}}}
\newcommand{\nsub}{\ensuremath{\tau_{32}^{\text{wta}}}}
\newcommand{\lumi}{\ensuremath{20.3~\ifb{}}}
\def\etconetwenty{\ensuremath{E_{T}^{0.2}}}
\def\etconethirty{\ensuremath{E_{T}^{0.3}}}
\def\ptconethirty{\ensuremath{p_{T}^{0.3}}}
\newcommand{\mymet}   {\ensuremath{E_{\mathrm{T}}^{\mathrm{miss}}}}
\newcommand{\etmiss}{$E_{\mathrm{T}}^{\mathrm{miss}}$}
%hypenated typewriter fonts 
% (see 
% http://tex.stackexchange.com/questions/44361/how-to-automatically-hyphenate-within-texttt )
\newcommand\hyptexttt[1]{\texttt{\hyphenchar\font=45\relax #1}}
% % Sub/superscript roman not italic (EE)
\def\MEX{\ensuremath{E_{\mathrm{x}}^{\mathrm{miss}}}}
\def\mex{\ensuremath{E_{\mathrm{x}}^{\mathrm{miss}}}}
\def\MEY{\ensuremath{E_{\mathrm{y}}^{\mathrm{miss}}}}
\def\mey{\ensuremath{E_{\mathrm{y}}^{\mathrm{miss}}}}
\def\MEXY{\ensuremath{E_{\mathrm{x,y}}^{\mathrm{miss}}}}
\def\mexy{\ensuremath{E_{\mathrm{x,y}}^{\mathrm{miss}}}}
\def\MEXYTRUTH{\ensuremath{E_{\mathrm{x,y Truth}}^{\mathrm{miss}}}}
\def\mexytruth{\ensuremath{E_{\mathrm{x,y Truth}}^{\mathrm{miss}}}}
\def\METTRUTH{\ensuremath{E_{\mathrm{T Truth}}^{\mathrm{miss}}}}
\def\mettruth{\ensuremath{E_{\mathrm{T Truth}}^{\mathrm{miss}}}}
% generators and formatting
\newcommand{\formatGenerator}[1]{\textsc{#1}}
\newcommand{\herwig}{{\sc Herwig}}
\newcommand{\powheg}{{\sc Powheg}}
\newcommand{\mcatnlo}{\formatGenerator{mcatnlo}}
\newcommand{\pythia}{{\sc Pythia}}
\newcommand{\pythiaSix}{\formatGenerator{pythia~6}}
\newcommand{\alpgen}{\formatGenerator{alpgen}}
\newcommand{\athena}{\formatGenerator{athena}}
\newcommand{\mcnlo}{{\sc Mc@nlo}}
\newcommand{\sherpa}{\formatGenerator{sherpa}}
\newcommand{\acermc}{\formatGenerator{acermc}}
\newcommand{\protos}{\formatGenerator{protos}}
\newcommand{\geantFour}{\formatGenerator{geant4}}
\newcommand{\jimmy}{\formatGenerator{jimmy}}
\newcommand{\hathor}{\formatGenerator{hathor}}
\newcommand{\atlfastTwo}{\formatGenerator{atlfast2}}
\newcommand{\wikiPage}[1]{\texttt{#1} wiki page}
% samples
\newcommand{\ttH}{\ensuremath{t\bar{t}H}}
%\newcommand{\wjets}{\ensuremath{W+\mathrm{jets}}}
\newcommand{\wjets}{$W$+jets}

\newcommand{\wbb} {\ensuremath{Wb\bar{b}+{\rm jets}}}
\newcommand{\wcc} {\ensuremath{Wc\bar{c}+{\rm jets}}}
\newcommand{\wc} {\ensuremath{Wc+{\rm jets}}}
\newcommand{\wlight} {\ensuremath{W+{\rm light~jets}}}
%\newcommand{\zjets}{\ensuremath{Z+\mathrm{jets}}}
\newcommand{\zjets}{$Z$+jets}

% matrix method
\newcommand{\effFake}{\ensuremath{\epsilon_{\mathrm{fake}}}}
\newcommand{\effReal}{\ensuremath{\epsilon_{\mathrm{real}}}}
% Analysis variables
\newcommand{\qg}{\ensuremath{qg}}
\newcommand{\AC}{\ensuremath{\text{A}_{\text{C}}}}
\newcommand{\ACsub}[1]{\ensuremath{\text{A}_{\text{C}, #1}}}
\newcommand{\Et}{\ensuremath{E_{\text{T}}}}
\newcommand{\Am}{\ensuremath{\text{A}_{\text{m}}}}
\newcommand{\Adr}{\ensuremath{\text{A}_{\Delta\text{R}}}}
%\newcommand{\rcurs}{{\mbox{$\resizebox{.09in}{.08in}{\includegraphics[trim= 1em 0 14em 0,clip]{ScriptR}}$}}}
\newcommand{\rcurs}{\ensuremath{\text{A}_\text{r}}}
%\newcommand{\pT}{\ensuremath{p_{\text{T}}}} % already defined in atlasphysics.sty
\newcommand{\ptSub}[1]{\ensuremath{p_{\text{T} #1}}}
\newcommand{\ptSup}[1]{\ensuremath{p_{\text{T}}^{#1}}}
\newcommand{\ptEl}{\ensuremath{p_{\text{T}}^{e}}}
\newcommand{\ptMu}{\ensuremath{p_{\text{T}}^{\mu{}}}}
%\newcommand{\met}{\ensuremath{\cancel{E}_{\text{T}}}} % already defined atlasphysics.sty
\newcommand{\mt}{\ensuremath{M_{\text{T}}}}
%\newcommand{\mtw}{\ensuremath{M_{\text{T,W}}}}
%\newcommand{\ttbar}{\ensuremath{t\bar{t}}} % already defined atlasphysics.sty
\newcommand{\TTbar}{\ensuremath{T\bar{T}}}
\newcommand{\Zprime}{\ensuremath{Z^\prime}}
\newcommand{\ttbarV}{\ensuremath{t\bar{t}+V}}
%\newcommand{\HT}{\ensuremath{H_{\text{T}}}} % already defined
\newcommand{\ST}{\ensuremath{S_{\text{T}}}}
\newcommand{\mtt}{\ensuremath{m_{\ttbar{}}}}
\newcommand{\pttt}{\ensuremath{p_{\text{T},\ttbar{}}}}
\newcommand{\ytt}{\ensuremath{y_{\ttbar{}}}}
\newcommand{\absYtt}{\ensuremath{\abs{y_{\ttbar{}}}}}
\newcommand{\betatt}{\ensuremath{\beta_{z,\ttbar{}}}}
\newcommand{\pp}{\ensuremath{pp}}
%\newcommand{\ppbar}{\ensuremath{p\bar{p}}}
\newcommand{\deltaR}[2]{\ensuremath{\Delta{}R\left(#1, #2\right)}}
% FBU-related
\providecommand{\abs}[1]{\lvert#1\rvert} 
\newcommand{\dy}{\ensuremath{\Delta{}\abs{y}}}
\newcommand{\diffVar}{\ensuremath{\varv{}}}
\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\thetavec}{\ensuremath{\vect{\theta{}}}}
\newcommand{\Truth}{\ensuremath{\vect{T}}}
\newcommand{\Data}{\ensuremath{\vect{D}}}
\newcommand{\Bckg}{\ensuremath{\vect{B}}}
\newcommand{\Reco}{\ensuremath{\vect{R}}}
\newcommand{\TrasfMatrix}{\ensuremath{\mathcal{M}}}
\newcommand{\Real}{\ensuremath{\mathbb{R}}}
\newcommand{\Integer}{\ensuremath{\mathbb{N}}}
\newcommand{\conditionalProb}[2]{\ensuremath{p\left(#1|#2\right)}}
\newcommand{\conditionalLhood}[2]{\ensuremath{\mathcal{L}\left(#1|#2\right)}}
\newcommand{\prior}{\ensuremath{\pi{}\left(\Truth{}\right)}}
\newcommand{\Tinf}{\ensuremath{T\ulcorner{}}}
\newcommand{\Tsup}{\ensuremath{T\urcorner{}}}
\DeclareMathOperator{\Erf}{Erf}
%------------
% other various commands
%------------
%
% redefine marginpar (with tighter spacing)
\let\oldmarginpar\marginpar
\renewcommand\marginpar[1]{
  \-\oldmarginpar[\raggedleft\footnotesize #1]{\raggedright\footnotesize #1}
}
% two types of margin notes
%\newcommand{\todo}[1]{\marginpar{{\scriptsize #1 }}}

%------------
%
%------------


==> journal/Makefile <==
# Makefile for creating an ATLAS paper draft using journal classes

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf
OPEN     = open

TEXFILES = $(wildcard *.tex)

.PHONY: texlive clean

all: atlas-elsevier atlas-jhep atlas-revtex

texlive:
	for file in $(TEXFILES); do \
	  if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	    echo "Changing texlive value in $$file"; \
	    sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $$file; \
	  else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \
	done

atlas-elsevier: atlas-elsevier.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jhep: atlas-jhep.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-revtex: atlas-revtex.pdf
	@echo "Made $<"
	# $(OPEN) $<

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Standard LaTeX targets
%.pdf: %.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.dvi: $(BASENAME).tex
	$(LATEX)    $<
	$(LATEX)    $<

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf \
	 *.spl *-revtexNotes.bib *.run.xml *.synctex.gz *~

cleanall: clean
	-rm *.pdf


==> journal/atlas-document-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

%% Title
\AtlasTitle{A simple ATLAS paper draft}
%
% Author - this does not work with revtex
% \author{The ATLAS Collaboration}
%
% Date: if not given, uses current date
% \date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{1.0}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GROUP-2014-XX}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2014-XXX}
% \AtlasNote{ATLAS-PUB-2014-XXX}
\AtlasNote{ATLAS-COM-PHYS-2014-XXX}

% Submission journal
\AtlasJournal{Phys.\ Lett.\ B.}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
	This is a bare bones ATLAS document used to demonstrate how to use journal templates.

	This document is typeset using the \DocumentStyle.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% Explicit list of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{A supporting note}{http://cds.cern.ch/record/XXXXXX}
\AtlasCoverSupportingNote{Another supporting note}{http://cds.cern.ch/record/YYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{DD Month 2014}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
\AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-GROUP-2014-XX-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-GROUP-2014-XX-editorial-board@cern.ch}

% CERN preprintnumber
\PreprintIdNumber{CERN-PH-2014-XX}

